Mind the Gap: The Difference Between Coverage and Mutation Score Can Guide Testing Efforts

An "adequate" test suite should effectively find all inconsistencies between a system's requirements/specifications and its implementation. Practitioners frequently use code coverage to approximate adequacy, while academics argue that mutation score may better approximate true (oracular) adequacy coverage. High code coverage is increasingly attainable even on large systems via automatic test generation, including fuzzing. In light of all of these options for measuring and improving testing effort, how should a QA engineer spend their time? We propose a new framework for reasoning about the extent, limits, and nature of a given testing effort based on an idea we call the oracle gap, or the difference between source code coverage and mutation score for a given software element. We conduct (1) a large-scale observational study of the oracle gap across popular Maven projects, (2) a study that varies testing and oracle quality across several of those projects and (3) a small-scale observational study of highly critical, well-tested code across comparable blockchain projects. We show that the oracle gap surfaces important information about the extent and quality of a test effort beyond either adequacy metric alone. In particular, it provides a way for practitioners to identify source files where it is likely a weak oracle tests important code.

==> Makefile <==
# Set this to the basename of the .tex file
# This will also be the name of the generated .dvi, .ps and .pdf files
PAPER = main

.PHONY: $(PAPER).pdf all clean

# Set this to the other source files that should be counted as
# dependencies
OTHERSOURCES := bibliography.bib \
	acmart.bib \
	$(filter-out $DOC, $(wildcard *.tex))

all: $(PAPER).pdf 


tidy:
	rm -rf *.aux *.out *.bbl *.toc *.log *.blg *.pyg *.cpt _minted*

# Using latexmk to generate the PDF
$(PAPER).pdf: $(PAPER).tex $(OTHERSOURCES)
	latexmk -pdf -pdflatex="pdflatex -interaction=nonstopmode" -use-make $(PAPER).tex

clean: tidy
	latexmk -CA


==> cut-tables.tex <==

\begin{table*}[ht]
\caption{Synthetic experiment corpus, consisting of 25 well-tested Java files
  over 5 projects.\label{tab:syntheticstats}}
\small
\centering
\begin{tabular}{llrrrrr}
\toprule
\bf Project               & \bf File                                      & \bf LOC & \bf \# Mutants & \bf \# Tests & \bf \# Asserts & \bf \# Asserts/Test \\
\midrule
\multirow{5}{*}{datasketches-java}         & DirectQuickSelectSketchTest.java              & 683  & 366        & 22       & 151        & 6.86            \\
                          & ReservoirItemsSketchTest.java                 & 458  & 604        & 14       & 85         & 6.07            \\
                          & UtilTest.java                                 & 279  & 1133       & 17       & 74         & 4.35            \\
                          & BoundsOnBinomialProportionsTest.java          & 104  & 702        & 4        & 12         & 3.00            \\
                          & MurmurHash3AdaptorTest.java                   & 297  & 741        & 17       & 53         & 3.12            \\
\midrule
\multirow{5}{*}{apollo}                    & StubClientTest.java                           & 242  & 44         & 17       & 24         & 1.41            \\
                          & JsonSerializerMiddlewaresTest.java            & 70   & 10         & 5        & 9          & 1.80            \\
                          & RuleRouterTest.java                           & 273  & 53         & 29       & 60         & 2.07            \\
                          & HeadersTest.java                              & 102  & 35         & 9        & 21         & 2.33            \\
                          & ServiceImplTest.java                          & 531  & 259        & 41       & 77         & 1.88            \\
\midrule
\multirow{5}{*}{lmdbjava}                  & CursorIterableTest.java                       & 271  & 51         & 21       & 47         & 2.24            \\
                          & KeyRangeTest.java                             & 233  & 35         & 19       & 41         & 2.16            \\
                          & ByteBufferProxyTest.java                      & 118  & 187        & 7        & 11         & 1.57            \\
                          & ResultCodeMapperTest.java                     & 124  & 32         & 5        & 7          & 1.40            \\
                          & TxnTest.java                                  & 257  & 113        & 7        & 19         & 2.71            \\
\midrule
\multirow{5}{*}{github-api}                & GHGistTest.java                               & 100  & 51         & 3        & 45         & 15.00           \\
                          & GHLicenseTest.java                            & 120  & 29         & 10       & 40         & 4.00            \\
                          & GHCheckRunBuilderTest.java                    & 114  & 131        & 6        & 23         & 3.83            \\
                          & GHWorkflowTest.java                           & 122  & 44         & 5        & 22         & 4.40            \\
                          & GHBranchProtectionTest.java                   & 87   & 14         & 6        & 18         & 3.00            \\
\midrule
\multirow{5}{*}{shardingsphere-elasticjob} & ElasticJobExecutorTest.java                   & 205  & 69         & 8        & 20         & 2.50            \\
                          & ShardingServiceTest.java                      & 246  & 146        & 18       & 37         & 2.06            \\
                          & AverageAllocationJobShardingStrategyTest.java & 56   & 88         & 6        & 6          & 1.00            \\
                          & AppConstraintEvaluatorTest.java               & 146  & 127        & 7        & 15         & 2.14            \\
                          & TaskContextTest.java                          & 92   & 110        & 13       & 27         & 2.08            \\

\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[ht]
  \caption{Comparison of synthetic experiment oracle gaps vs. descartes pseudotesting scores.\label{tab:descartes}}
  \small
  \centering
  \begin{tabular}{llrrrr}
  \toprule
  \bf Project               & \bf File                                      & \bf Pseudo \% & \bf Covered Mut. Score & \bf Covered Gap & \bf Pseudo Gap \\
  \midrule
  \multirow{5}{*}{datasketches-java}         
                            & DirectQuickSelectSketch.java              & 100\%    & 61.3\%     & 34.1\%       & -4.6\%         \\
                            & ReservoirItemsSketch.java                 & 96\% & 68.5\%     & 30.2\%   & 2.7\%      \\
                            & Util.java                                 & 93\% & 73.4\%     & 25.0\%   & 5.4\%      \\
                            & BoundsOnBinomialProportions.java          & 100\% & 92.0\%    & 8.5\%    & 0.5\%      \\
                            & MurmurHash3Adaptor.java                   & 74\%  & 50.7\%    & 48.0\%   & 24.7\%     \\
  \midrule 
  \multirow{5}{*}{apollo}                    
                            & StubClient.java                           & 88\%     & 66.7\%     & 26.1\%       & 4.8\%           \\
                            & JsonSerializerMiddlewares.java            & 100\% & 100\%     & -5.0\%   & -5.0\%     \\
                            & RuleRouter.java                           & 100\% & 91.4\%    & -18.9\%  & -27.5\%    \\
                            & Headers.java                              & 100\% & 83.9\%    & 16.1\%   & 0.0\%      \\
                            & ServiceImpl.java                          & 83\%  & 60.3\%    & 33.8\%   & 11.1\%     \\
  \midrule
  \multirow{5}{*}{lmdbjava}                  
                            & CursorIterable.java                       & 100\%    & 82.5\%     & 12.2\%       & -5.3\%          \\
                            & KeyRange.java                             & 100\% & 77.8\%    & 22.2\%   & 0.0\%      \\
                            & ByteBufferProxy.java                      & 87\% & 76.4\%     & 15.1\%   & 4.5\%      \\
                            & ResultCodeMapper.java                     & 100\% & 96.2\%    & 3.8\%    & 0.0\%      \\
                            & Txn.java                                  & 100\% & 79.1\%    & 19.6\%   & -1.3\%     \\
  \midrule
  \multirow{5}{*}{github-api}                
                            & GHGist.java                               & 75\%     & 76.3\%     & 20.3\%       & 21.6\%          \\
                            & GHLicense.java                            & 86\% & 50.0\%     & 44.2\%   & 8.2\%      \\
                            & GHCheckRunBuilder.java                    & 100\% & 97.9\%    & -2.9\%   & -5.0\%     \\
                            & GHWorkflow.java                           & 80\% & 80.0\%     & 9.1\%    & 9.1\%      \\
                            & GHBranchProtection.java                   & 60\% & 50.0\%     & 21.2\%   & 11.2\%     \\
  \midrule
  \multirow{5}{*}{shardingsphere-elasticjob} 
                            & ElasticJobExecutor.java                   & 100\%    & 69.6\%     & 21.5\%       & -8.9\%          \\
                            & ShardingService.java                      & 85\% & 71.0\%     & 29.0\%   & 15.0\%     \\
                            & AverageAllocationJobShardingStrategy.java & 100\% & 88.8\%    & 11.3\%   & 0.1\%      \\
                            & AppConstraintEvaluator.java               & 100\% & 64.2\%    & 35.8\%  &  0.0\%      \\
                            & TaskContext.java                          & 100\% & 94.7\%    & 4.4\%   & -0.9\%      \\
  
  \bottomrule
  \end{tabular}
  \end{table*}


\begin{table*}
  \caption{Table of various terms introduced throughout the paper and their formulas.}
  \centering
  \begin{tabular}{ll}
  \toprule
  \bf Metric                   & \bf Formula                 \\                                     
  \midrule
  Oracle gap                      & coverage - mutation score \\                                       
  Covered oracle gap              & coverage - covered mutation score \\                                      
  Pseudo gap                      & coverage - covered pseudotesting score \\  
  Covered mutation score          & mutation score over covered lines \\                                           
  Covered pseudotesting score     & mutation score over covered pseudotesting mutants \\                                                                                    
  \bottomrule
  \end{tabular}
  \label{tab:metrics}
  \end{table*}
  

\begin{table*}
\caption{Descriptive Statistics for Large Java Corpus.}
% Files/project and lines of code/project are computed 
%for all files in the project. All other metrics are computed for sampled files
%only.}
% CLG thinks that's intuitive enough to save the space
\centering
\begin{tabular}{lrrrr|r}
\toprule
\bf Statistic                   & \bf Mean        & \bf Median    & \bf Range               & \bf Std. Dev.            & \bf Total    \\
\midrule
\#files/project                 & 267.8           & 156.0           & [2, 2667]               & 447.0                    & 12051.0        \\
%mutant runtime/project          & 3105.4          & 1815.4        & [2.81, 452998]          & 14196.0                  & 3285536.3    \\
mutant runtime/project (mins)   & 51.8            & 30.3          & [0.05, 7549.9]          & 236.6                    & 54758.9    \\
line coverage/file              & 63.8            & 81.3          & [0, 100]                & 39.5                     & -            \\
lines of code/project           & 10298.2         & 5767.0          & [18, 42774]             & 11715.0                  & 463417.0       \\
\# tests/project                & 1277.6          & 483.0           & [24, 8804]              & 1881.2                   & 42161.0        \\
\#mutants/file                  & 41.9            & 30.5          & [0, 99]                 & 36.0                     & 44320.0        \\

\bottomrule
\end{tabular}
\label{tab:corpus}
\end{table*}


==> old-intro.tex <==

Software engineers are well aware that executing code and testing code are not
actually the same, with research and practical literature both containing
numerous invocations of the distinction. The primary framework for this concept
is usually to distinguish tests from specifications, particularly, via the
notion of an oracle, which is central to both academic \cite{StaatsOracle} and
practical work on testing \cite{LessonsLearned}. Academic formulations of this
distinction range from foundational descriptions of how tests and oracles work
together in detecting faults \cite{StaatsOracle} to proposals for notions of
\emph{code coverage} that include more explicit determination of not just if
code is executed, but whether the code is \emph{checked} for correctness
\cite{ZellerCheckedCov}.

However, in practice, most notions of \emph{testedness} used in
real-world software testing, and, critically, even in research, conflate the two
concepts.  The vast majority of projects that quantitatively evaluate
tested code rely on source code coverage, either statement or
branch coverage~\cite{Discontents}. Source code coverage essentially
ignores the oracle question: executing all code while testing nothing
(or only that a program does not actually crash) is sufficient to
obtain good source code coverage. 
A much smaller number of projects use a mutation
score, a single value that is a summary of both coverage and oracle
power.  In neither case is the \emph{difference} between execution and
checking clear: the focus is on a number indicating a single ``degree
of testedness.''  

However, understanding that coverage is not a ``cheap and weak'' form
of mutation score, or mutation score a ``more precise'' coverage value
may be
essential for a better understanding of the true complexity of software testing.  Consider an
effort to \emph{fuzz} a highly critical software component.
Frequently, a fuzzing effort can achieve high code
coverage without being effective in detecting bugs that are not
crashes.  This is because fuzzing typically only detects crashes;
determining the correct behavior for random
inputs fuzzing produces is a hard problem.  In this case, a
large gap exists between source code coverage and the mutation score for that
code.  We refer to this as the \emph{oracle gap}.  Fuzzing inherently
tends towards a large oracle gap, and this is a key fact about the
nature and proper uses for fuzzing.

More precisely, we define the \emph{oracle gap} as \emph{the
  difference between source code coverage and mutation score for a
  given software element}.    Our
intuition is that raw oracle gaps are usually positive.
In general, source code coverage is usually higher 
than mutation score, since basic coverage is easier to achieve,
only in rare instances a small part of a program may contribute a
large number of mutants, and be well-checked, while much of the rest
of the code is not tested --- code not covered will obviously also produce mutants that are not detected. More common, however, is the case where a
testing effort (in our example, fuzzing) has high code coverage but a
low mutation score, resulting in a large oracle gap.  This means that
the most effective way to improve a testing effort's fault detection ability
would be to improve the oracle, rather than to execute more code.
The utility of the oracle gap derives from the fact that, in fuzzing,
improving coverage will almost always be \emph{easier} than improving the
oracle, so only in the context of a large gap is oracle improvement
likely to be cost-effective.

In this paper, we argue that the oracle gap is a useful and effective idea for
understanding and potentially operationalizing existing, long-standing test adequacy metrics.  The
oracle gap will only grow in importance as automated generation of
tests becomes more important, whether by fuzzing or other means.

